Directional Variance Adjustment: improving covariance estimates for high-dimensional portfolio optimization

Robust and reliable covariance estimates play a decisive role in financial and many other applications. An important class of estimators is based on Factor models. Here, we show by extensive Monte Carlo simulations that covariance matrices derived from the statistical Factor Analysis model exhibit a systematic error, which is similar to the well-known systematic error of the spectrum of the sample covariance matrix. Moreover, we introduce the Directional Variance Adjustment (DVA) algorithm, which diminishes the systematic error. In a thorough empirical study for the US, European, and Hong Kong market we show that our proposed method leads to improved portfolio allocation.

==> source/furthersims.tex <==
%!TEX root = /Users/danielbartz/dbmlu/publications/papers/2012_01_DVA_revision2/JoCSaDA_DVA.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We expect that the systematic error might get larger when kurtosis increases because estimation gets more difficult when the influence of rare events gets larger. We start again by looking at the empirical eigenvalue distribution of sample covariance matrices for different sample sizes. For this, we generate artificial data from t-distributions. The t-distribution's variance $\sigma_t$ and kurtosis $k_t$ depend on its degrees of freedom $\nu$,
$$
\sigma_t^2 = \frac{\nu}{\nu-2} \quad \mathrm{for} \quad \nu>2, \qquad k_t = \frac{\nu}{\nu-4} \quad \mathrm{for} \quad \nu>4.
$$
Therefore, we can generate a t-distribution with arbitrary kurtosis $k_g$ and variance $\sigma_g^2$ by setting the degrees of freedom to
\begin{align}
\nu_g = \frac{6}{k_g} + 4 \label{eq:dfkurt}
\end{align}
and rescaling appropriately. In \cite{Lon05}, it is shown that asset returns have the same tail behaviour as t-distributions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulation Results for DVA Factor Analysis}
\label{app:fasc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Results for simulations  with data generated according to the scheme presented in section \ref{sec:fabias} are shown in Figure~\ref{fig:bcfadw}. The  DVA method reduces the systematic error towards zero in the majority of the space orthogonal to the factors. In the factor subspace and for the eigendirections corresponding to the smallest eigenvalues the systematic error is reduced strongly. 
%The results for subspacewise correction are not as good. The high difference in bias of the more and less pronounced factors cannot be accounted for. The bias in the variances of the orthogonal complement, which is, as mentioned above, similar to the bias in the eigenvalues of the sample covariance matrix, cannot be corrected for neither. This leads to a remaining upwards bias of the large variances and a downwards bias of  the small ones. Note that the differences through bias correction are just paralell shifts in the log plot for each of the two subspaces. Due to the superiority of the dimensionwise approach, in the following the subspacewise method will not be investigated further.
\begin{figure} 
\begin{center}
\includegraphics[width=12cm]{images/bcfadw.pdf}
\caption{comparison of the systematic error of DVA and standard Factor Analysis. Correction factors estimated on $ K=100 $ generated data sets. Mean over 150 simulations. Sample Size $T=150$.} \label{fig:bcfadw}
% generated with techFMbiascorrdw
\end{center}
\end{figure}


